Calculations for deep inelastic scattering using fast interpolation grid techniques at NNLO in QCD and the extraction of $\alpha_s$ from HERA data

The extension of interpolation-grid frameworks for perturbative QCD calculations at next-to-next-to-leading order (NNLO) is presented for deep inelastic scattering (DIS) processes. A fast and flexible evaluation of higher-order predictions for any a posteriori choice of parton distribution functions (PDFs) or value of the strong coupling constant is essential in iterative fitting procedures to extract PDFs and Standard Model parameters as well as for a detailed study of the scale dependence. The APPLfast project, described here, provides a generic interface between the parton-level Monte Carlo program NNLOJET and both the APPLgrid and fastNLO libraries for the production of interpolation grids at NNLO accuracy. Details of the interface for DIS processes are presented together with the required interpolation grids at NNLO, which are made available. They cover numerous inclusive jet measurements by the H1 and ZEUS experiments at HERA. An extraction of the strong coupling constant is performed as an application of the use of such grids and a best-fit value of $\alpha_s(M_Z) = 0.1178\,(15)_\text{exp}\,(21)_\text{th}$ is obtained using the HERA inclusive jet cross section data.

==> makefile <==

SOURCE = applfast.tex       \
	tex/abs.tex         \
	tex/intro.tex       \
	tex/internals.tex   \
	tex/applfastproj.tex       \
	tex/analysis.tex    \
	tex/conclusions.tex \
	tex/ack.tex

all:  new erratum short diff

#applfast: $(SOURCE)
new: $(SOURCE)
	pdflatex applfast.tex
	bibtex applfast
	pdflatex applfast.tex
	pdflatex applfast.tex

erratum: $(SOURCE)
	pdflatex applfast_erratum.tex
	bibtex applfast_erratum
	pdflatex applfast_erratum.tex
	pdflatex applfast_erratum.tex

short: $(SOURCE)
	pdflatex applfast_short_erratum.tex
	bibtex applfast_short_erratum
	pdflatex applfast_short_erratum.tex
	pdflatex applfast_short_erratum.tex

diff:
	tar -xzf arXiv_v2.tar.gz
	latexdiff --flatten applfast_v2.tex applfast.tex > diff-applfast.tex
	pdflatex diff-applfast.tex
#	bibtex   diff-applfast
	pdflatex diff-applfast.tex
	pdflatex diff-applfast.tex

clean :
	rm -f *.aux *.bbl *.blg *.dvi *.log *.out *.toc

